Loop Equations for Multi-Matrix Models

We revisit the combinatorial loop-equation method for computing planar disc amplitudes in multi-matrix models with polynomial potentials. We develop a procedure which organises the Schwinger-Dyson constraints by the level of their boundary insertions and, when the resulting system closes, produces an algebraic equation for the planar disc function. Using this method we recover the disc partition functions associated with fixed, mixed, and free boundary conditions in the three-state Potts model, previously obtained by saddle-point methods. As a novelty we derive an algebraic equation for the fixed-boundary resolvent of the three-state Potts model with unequal quadratic and cubic couplings. We further show one can compute the disc partition function for several unsolved two- and three-matrix models. These examples demonstrate that loop equations provide a practical route to identifying and solving sectors of multi-matrix models beyond the standard one- and two-matrix cases.

==> text/asymptotics/quartic_mgg.tex <==
% Generated by scripts/format_sheet_expansions.py.
% Original potential parameters; no displayed coefficient abbreviations.
% Terms through z^{-1}; deeper moments remain in the source series.
\begin{sheetasymptotics}
    \begin{align*}
        \sheetlabel{W_A(z)_{0}} & ={}z^{-1}+\mathcal O(z^{-2}) \\[4pt]
        \sheetlabel{W_A(z)_{1}} & ={}-gz^{3}+z+z^{-1}+\mathcal O(z^{-2}) \\[4pt]
        \sheetlabel{W_A(z)_{2}} & ={}3z-z^{-1}+\mathcal O(z^{-2}) \\[4pt]
        \sheetlabel{W_A(z)_{3}} & ={}4z-\frac{2 \sqrt[3]{2}}{\sqrt[3]{g}}z^{1/3}+\frac{2^{2/3}}{g^{2/3}}z^{-1/3}-\frac{1}{3}z^{-1}+\mathcal O(z^{-5/3}) \\[4pt]
        \sheetlabel{W_A(z)_{4}} & ={}4z+\frac{\sqrt[3]{2} \left(1 - i \sqrt{3}\right)}{\sqrt[3]{g}}z^{1/3}+\frac{2^{2/3} \left(- \frac{1}{2} - \frac{i \sqrt{3}}{2}\right)}{g^{2/3}}z^{-1/3}-\frac{1}{3}z^{-1}+\mathcal O(z^{-5/3}) \\[4pt]
        \sheetlabel{W_A(z)_{5}} & ={}4z+\frac{\sqrt[3]{2} \left(1 + i \sqrt{3}\right)}{\sqrt[3]{g}}z^{1/3}+\frac{2^{2/3} \left(- \frac{1}{2} + \frac{i \sqrt{3}}{2}\right)}{g^{2/3}}z^{-1/3}-\frac{1}{3}z^{-1}+\mathcal O(z^{-5/3})
    \end{align*}
\end{sheetasymptotics}


==> text/curves/dilute_fixed.tex <==
% Generated from notebooks/Dilute Potts Fixed.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:dilute_fixed}
    F_{(1)}(x,y)={} & \frac{4 t_0^4}{t_3}y^{9}{}+y^{8}\left(-32 t_0^4x^{2} - \frac{32 t_0^4 t_2}{t_3}x - \frac{16 t_0^3}{t_3}\right)\notag \\
                    & {}+y^{7}\left(112 t_0^4 t_3x^{4} + 224 t_0^4 t_2x^{3} + \frac{112 t_0^3 \left(t_0 t_2^2+t_3\right)}{t_3}x^{2} + \frac{4 t_0^3 \left(28 t_2+t_0 t_3-3\right)}{t_3}x\right.\notag \\*
                    & \qquad{}\left.{}+ c_{0,7}\right)\notag \\
                    & {}+y^{6}\left(-224 t_0^4 t_3^2x^{6} - 672 t_0^4 t_2 t_3x^{5} - 336 t_0^3 \left(2 t_0 t_2^2+t_3\right)x^{4}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{4 t_0^3 \left(56 t_0 t_2^3+168 t_3 t_2+7 t_0 t_3^2-18 t_3\right)}{t_3}x^{3} + \sum_{i=0}^{2}c_{i,6}x^i\right)\notag \\
                    & {}+y^{5}\left(280 t_0^4 t_3^3x^{8} + 1120 t_0^4 t_2 t_3^2x^{7} + 560 t_0^3 t_3 \left(3 t_0 t_2^2+t_3\right)x^{6}\right.\notag \\*
                    & \qquad{}\left.{}+ 4 t_0^3 \left(280 t_0 t_2^3+420 t_3 t_2+21 t_0 t_3^2-45 t_3\right)x^{5} + \sum_{i=0}^{4}c_{i,5}x^i\right)\notag \\
                    & {}+y^{4}\left(-224 t_0^4 t_3^4x^{10} - 1120 t_0^4 t_2 t_3^3x^{9} - 560 t_0^3 t_3^2 \left(4 t_0 t_2^2+t_3\right)x^{8}\right.\notag \\*
                    & \qquad{}\left.{}- 20 t_0^3 t_3 \left(112 t_0 t_2^3+112 t_3 t_2+7 t_0 t_3^2-12 t_3\right)x^{7} + \sum_{i=0}^{6}c_{i,4}x^i\right)\notag \\
                    & {}+y^{3}\left(112 t_0^4 t_3^5x^{12} + 672 t_0^4 t_2 t_3^4x^{11} + 336 t_0^3 t_3^3 \left(5 t_0 t_2^2+t_3\right)x^{10}\right.\notag \\*
                    & \qquad{}\left.{}+ 20 t_0^3 t_3^2 \left(112 t_0 t_2^3+84 t_3 t_2+7 t_0 t_3^2-9 t_3\right)x^{9} + \sum_{i=0}^{8}c_{i,3}x^i\right)\notag \\
                    & {}+y^{2}\left(-32 t_0^4 t_3^6x^{14} - 224 t_0^4 t_2 t_3^5x^{13} - 112 t_0^3 t_3^4 \left(6 t_0 t_2^2+t_3\right)x^{12}\right.\notag \\*
                    & \qquad{}\left.{}- 4 t_0^3 t_3^3 \left(280 t_0 t_2^3+168 t_3 t_2+21 t_0 t_3^2-18 t_3\right)x^{11} + \sum_{i=0}^{10}c_{i,2}x^i\right)\notag \\
                    & {}+y\left(4 t_0^4 t_3^7x^{16} + 32 t_0^4 t_2 t_3^6x^{15} + 16 t_0^3 t_3^5 \left(7 t_0 t_2^2+t_3\right)x^{14}\right.\notag \\*
                    & \qquad{}\left.{}+ 4 t_0^3 t_3^4 \left(56 t_0 t_2^3+28 t_3 t_2+7 t_0 t_3^2-3 t_3\right)x^{13} + \sum_{i=0}^{12}c_{i,1}x^i\right)\notag \\
                    & {}-4 t_0^4 t_3^7x^{15} + \sum_{i=0}^{14}c_{i,0}x^i.
\end{align}


==> text/curves/dilute_vacant.tex <==
% Generated from notebooks/Dilute Potts Absent.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:dilute_vacant}
    F(x,y)={} & \frac{1}{t_0}y^{6}{}+y^{5}\left(-12x^{2} - \frac{12}{t_0}x - \frac{18 t_2}{t_0 t_3}\right)\notag \\
              & {}+y^{4}\left(54 t_0x^{4} + 108x^{3} + \frac{54 \left(3 t_0 t_2+t_3\right)}{t_0 t_3}x^{2} + \frac{6 \left(27 t_2+t_0 t_3-3\right)}{t_0 t_3}x + c_{0,4}\right)\notag \\
              & {}+y^{3}\left(-112 t_0^2x^{6} - 336 t_0x^{5} - \frac{168 \left(3 t_0 t_2+2 t_3\right)}{t_3}x^{4}\right.\notag \\*
              & \qquad{}\left.{}- \frac{16 \left(3 t_3 t_0^2+63 t_2 t_0-9 t_0+7 t_3\right)}{t_0 t_3}x^{3} + \sum_{i=0}^{2}c_{i,3}x^i\right)\notag \\
              & {}+y^{2}\left(105 t_0^3x^{8} + 420 t_0^2x^{7} + \frac{630 t_0 \left(t_0 t_2+t_3\right)}{t_3}x^{6}\right.\notag \\*
              & \qquad{}\left.{}+ \frac{42 \left(3 t_3 t_0^2+45 t_2 t_0-9 t_0+10 t_3\right)}{t_3}x^{5} + \sum_{i=0}^{4}c_{i,2}x^i\right)\notag \\
              & {}+y\left(-36 t_0^4x^{10} - 180 t_0^3x^{9} - \frac{90 t_0^2 \left(3 t_0 t_2+4 t_3\right)}{t_3}x^{8}\right.\notag \\*
              & \qquad{}\left.{}- \frac{120 t_0 \left(t_3 t_0^2+9 t_2 t_0-3 t_0+3 t_3\right)}{t_3}x^{7} + \sum_{i=0}^{6}c_{i,1}x^i\right)\notag \\
              & {}+36 t_0^4x^{9} + \sum_{i=0}^{8}c_{i,0}x^i.
\end{align}


==> text/curves/ising_fixed.tex <==
% Generated from notebooks/Dilute Ising Fixed.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:ising_fixed}
    F_{(1)}(x,y)={} & -t_0y^{5}{}+y^{4}\left(4 t_0 t_3x^{2} + 4 t_0 t_2x + 2\right)\notag \\
                    & {}+y^{3}\left(-6 t_0 t_3^2x^{4} - 12 t_0 t_2 t_3x^{3} - 6 \left(t_0 t_2^2+t_3\right)x^{2} + \bigl(-6 t_2-t_0 t_3+2\bigr)x + c_{0,3}\right)\notag \\
                    & {}+y^{2}\left(4 t_0 t_3^3x^{6} + 12 t_0 t_2 t_3^2x^{5} + 6 t_3 \left(2 t_0 t_2^2+t_3\right)x^{4}\right.\notag \\*
                    & \qquad{}\left.{}+ \bigl(4 t_0 t_2^3+12 t_3 t_2+3 t_0 t_3^2-4 t_3\bigr)x^{3} + \sum_{i=0}^{2}c_{i,2}x^i\right)\notag \\
                    & {}+y\left(-t_0 t_3^4x^{8} - 4 t_0 t_2 t_3^3x^{7} - 2 t_3^2 \left(3 t_0 t_2^2+t_3\right)x^{6}\right.\notag \\*
                    & \qquad{}\left.{}- t_3 \left(4 t_0 t_2^3+6 t_3 t_2+3 t_0 t_3^2-2 t_3\right)x^{5} + \sum_{i=0}^{4}c_{i,1}x^i\right)\notag \\
                    & {}+t_0 t_3^4x^{7} + \sum_{i=0}^{6}c_{i,0}x^i.
\end{align}


==> text/curves/ising_free.tex <==
% Generated from notebooks/Dilute Ising Free.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:ising_free}
    F_{(2)}(x,y)={} & -\frac{256 t_0^2}{t_3^2}y^{10}{}+y^{9}\left(\frac{256 t_0^2}{t_3}x^{2} + \frac{512 t_0^2 t_2}{t_3^2}x + \frac{512 t_0}{t_3^2}\right)\notag \\
                    & {}+y^{8}\left(-96 t_0^2x^{4} - \frac{384 t_0^2 t_2}{t_3}x^{3} - \frac{384 t_0 \left(t_0 t_2^2+t_3\right)}{t_3^2}x^{2} - \frac{768 t_0 t_2}{t_3^2}x + c_{0,8}\right)\notag \\
                    & {}+y^{7}\left(16 t_0^2 t_3x^{6} + 96 t_0^2 t_2x^{5} + \frac{96 t_0 \left(2 t_0 t_2^2+t_3\right)}{t_3}x^{4} + \frac{128 t_0 t_2 \left(t_0 t_2^2+3 t_3\right)}{t_3^2}x^{3}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{2}c_{i,7}x^i\right)\notag \\
                    & {}+y^{6}\left(-t_0^2 t_3^2x^{8} - 8 t_0^2 t_2 t_3x^{7} - 8 t_0 \left(3 t_0 t_2^2+t_3\right)x^{6} - \frac{16 t_0 t_2 \left(2 t_0 t_2^2+3 t_3\right)}{t_3}x^{5}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{4}c_{i,6}x^i\right)\notag \\
                    & {}+\sum_{i=0}^{6}c_{i,5}x^iy^{5}\notag \\
                    & {}+y^{4}\left(-\left(\left(4 t_0 t_2-t_3\right) t_3\right)x^{8} - 8 t_2 \left(4 t_0 t_2-t_3\right)x^{7} + \sum_{i=0}^{6}c_{i,4}x^i\right)\notag \\
                    & {}+y^{3}\left(64 t_3x^{8} + 512 t_2x^{7} + \sum_{i=0}^{6}c_{i,3}x^i\right)\notag \\
                    & {}+y^{2}\left(-4 t_3^2x^{10} - 40 t_2 t_3x^{9} + \sum_{i=0}^{8}c_{i,2}x^i\right)\notag \\
                    & {}+\sum_{i=0}^{8}c_{i,1}x^iy\notag \\
                    & {}+4 t_3^2x^{8} + 32 t_2 t_3x^{7} + \sum_{i=0}^{6}c_{i,0}x^i.
\end{align}


==> text/curves/ising_vacant.tex <==
% Generated from notebooks/Dilute Ising Absent.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:ising_vacant}
    F(x,y)={} & -\frac{1}{4 t_0}y^{4}{}+y^{3}\left(x^{2} + \frac{1}{t_0}x + \frac{t_2}{t_0 t_3}\right)\notag \\
              & {}+y^{2}\left(-\frac{5 t_0}{4}x^{4} - \frac{5}{2}x^{3} - \frac{5 \left(2 t_0 t_2+t_3\right)}{4 t_0 t_3}x^{2} - \frac{5 t_2+t_0 t_3-2}{2 t_0 t_3}x + c_{0,2}\right)\notag \\
              & {}+y\left(\frac{t_0^2}{2}x^{6} + \frac{3 t_0}{2}x^{5} + \frac{3 \left(t_0 t_2+t_3\right)}{2 t_3}x^{4} + \frac{2 t_3 t_0^2+6 t_2 t_0-4 t_0+t_3}{2 t_0 t_3}x^{3} + \sum_{i=0}^{2}c_{i,1}x^i\right)\notag \\
              & {}-\frac{t_0^2}{2}x^{5} + \sum_{i=0}^{4}c_{i,0}x^i.
\end{align}


==> text/curves/potts_general_full.tex <==
% Generated from notebooks/asymmetric_potts_fixed.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:potts_general_full}
    F_{(1)}(x,y)={} & y^{7}{}+y^{6}\left(-t_3x^{2} + \bigl(-t_2-5\bigr)x\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{2 r_3 s_3 t_2+12 r_2 s_3 t_3+12 r_3 s_2 t_3-r_3 s_3-8 r_3 t_3-8 s_3 t_3}{4 r_3 s_3 t_3}\right)\notag \\
                    & {}+y^{5}\left(5 t_3x^{3} + \frac{9 r_3 s_3 t_2-6 r_2 s_3 t_3-6 r_3 s_2 t_3+21 r_3 s_3+4 r_3 t_3+4 s_3 t_3}{2 r_3 s_3}x^{2}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{\begin{gathered}
                                                r_3 s_3 t_2^2 +4 r_3 s_3 t_2 +6 r_3 s_2 t_3 t_2 +6 r_2 s_3 t_3 t_2 -2 r_3 s_3 t_3^2 \\
                                                +25 r_3 s_2 t_3 +25 r_2 s_3 t_3 -2 r_3 s_3 -4 r_3 t_3 t_2 -12 r_3 t_3 -4 s_3 t_3 t_2 \\
                                                -12 s_3 t_3
                                            \end{gathered}}{2 r_3 s_3 t_3}x\right.\notag \\*
                    & \qquad{}\left.{}+ c_{0,5}\right)\notag \\
                    & {}+y^{4}\left(-\frac{41 t_3}{4}x^{4}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{16 r_3 s_3 t_2-25 r_2 s_3 t_3-25 r_3 s_2 t_3+24 r_3 s_3+12 r_3 t_3+12 s_3 t_3}{2 r_3 s_3}x^{3}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{\begin{gathered}
                                                9 r_3^2 s_3^2 t_2^2 -13 r_3^2 s_2^2 t_3^2 -18 r_3^2 s_3^2 t_3^2 +16 r_3^2 s_2 t_3^2 \\
                                                +12 r_3^2 s_3^2 t_2 +84 r_3^2 s_2 s_3 t_3 -28 r_3^2 s_3 t_3 +45 r_3^2 s_2 s_3 t_2 t_3 \\
                                                -20 r_3^2 s_3 t_2 t_3 +16 r_2 r_3 s_3 t_3^2 -30 r_2 r_3 s_2 s_3 t_3^2 +16 r_3 s_2 s_3 t_3^2 \\
                                                +8 r_3 s_3 t_3^2 +84 r_2 r_3 s_3^2 t_3 -28 r_3 s_3^2 t_3 +45 r_2 r_3 s_3^2 t_2 t_3 \\
                                                -20 r_3 s_3^2 t_2 t_3 -13 r_2^2 s_3^2 t_3^2 +16 r_2 s_3^2 t_3^2 -6 r_3^2 s_3^2 \\
                                                -4 r_3^2 t_3^2 -4 s_3^2 t_3^2
                                            \end{gathered}}{4 r_3^2 s_3^2 t_3}x^{2} + c_{1,4}x\right.\notag \\*
                    & \qquad{}\left.{}+ c_{0,4}\right)\notag \\
                    & {}+y^{3}\left(11 t_3x^{5}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{14 r_3 s_3 t_2-41 r_2 s_3 t_3-41 r_3 s_2 t_3+16 r_3 s_3+13 r_3 t_3+13 s_3 t_3}{2 r_3 s_3}x^{4}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{\begin{gathered}
                                                4 r_3^2 s_3^2 t_2^2 -11 r_3^2 s_2^2 t_3^2 -8 r_3^2 s_3^2 t_3^2 +9 r_3^2 s_2 t_3^2 \\
                                                +2 r_3^2 s_3^2 t_2 +18 r_3^2 s_2 s_3 t_3 -4 r_3^2 s_3 t_3 +16 r_3^2 s_2 s_3 t_2 t_3 \\
                                                -4 r_3^2 s_3 t_2 t_3 +9 r_2 r_3 s_3 t_3^2 -25 r_2 r_3 s_2 s_3 t_3^2 +9 r_3 s_2 s_3 t_3^2 \\
                                                +2 r_3 s_3 t_3^2 +18 r_2 r_3 s_3^2 t_3 -4 r_3 s_3^2 t_3 +16 r_2 r_3 s_3^2 t_2 t_3 \\
                                                -4 r_3 s_3^2 t_2 t_3 -11 r_2^2 s_3^2 t_3^2 +9 r_2 s_3^2 t_3^2 +r_3^2 \bigl( -s_3^2\bigr) \\
                                                -r_3^2 t_3^2 -s_3^2 t_3^2
                                            \end{gathered}}{r_3^2 s_3^2 t_3}x^{3}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{2}c_{i,3}x^i\right)\notag \\
                    & {}+y^{2}\left(-\frac{13 t_3}{2}x^{6}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{3 \left(2 r_3 s_3 t_2-11 r_2 s_3 t_3-11 r_3 s_2 t_3+2 r_3 s_3+2 r_3 t_3+2 s_3 t_3\right)}{2 r_3 s_3}x^{5}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{\begin{gathered}
                                                14 r_3^2 s_3^2 t_2^2 -55 r_3^2 s_2^2 t_3^2 -28 r_3^2 s_3^2 t_3^2 +26 r_3^2 s_2 t_3^2 \\
                                                +2 r_3^2 s_3^2 t_2 +32 r_3^2 s_2 s_3 t_3 -4 r_3^2 s_3 t_3 +42 r_3^2 s_2 s_3 t_2 t_3 \\
                                                -4 r_3^2 s_3 t_2 t_3 +26 r_2 r_3 s_3 t_3^2 -123 r_2 r_3 s_2 s_3 t_3^2 +26 r_3 s_2 s_3 t_3^2 \\
                                                +2 r_3 s_3 t_3^2 +32 r_2 r_3 s_3^2 t_3 -4 r_3 s_3^2 t_3 +42 r_2 r_3 s_3^2 t_2 t_3 \\
                                                -4 r_3 s_3^2 t_2 t_3 -55 r_2^2 s_3^2 t_3^2 +26 r_2 s_3^2 t_3^2 +r_3^2 \bigl( -s_3^2\bigr) \\
                                                -r_3^2 t_3^2 -s_3^2 t_3^2
                                            \end{gathered}}{4 r_3^2 s_3^2 t_3}x^{4}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{3}c_{i,2}x^i\right)\notag \\
                    & {}+y\left(2 t_3x^{7} + \frac{r_3 s_3 t_2-13 r_2 s_3 t_3-13 r_3 s_2 t_3+r_3 s_3+r_3 t_3+s_3 t_3}{2 r_3 s_3}x^{6}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{\begin{gathered}
                                                3 \bigl(r_3^2 \bigl( -s_3^2\bigr) t_2^2 +5 r_3^2 s_2^2 t_3^2 +2 r_3^2 s_3^2 t_3^2 -r_3^2 s_2 t_3^2 \\
                                                -r_3^2 s_2 s_3 t_3 -2 r_3^2 s_2 s_3 t_2 t_3 -r_2 r_3 s_3 t_3^2 +11 r_2 r_3 s_2 s_3 t_3^2 \\
                                                -r_3 s_2 s_3 t_3^2 -r_2 r_3 s_3^2 t_3 -2 r_2 r_3 s_3^2 t_2 t_3 +5 r_2^2 s_3^2 t_3^2 \\
                                                -r_2 s_3^2 t_3^2\bigr)
                                            \end{gathered}}{2 r_3^2 s_3^2 t_3}x^{5}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{4}c_{i,1}x^i\right)\notag \\
                    & {}-\frac{t_3}{4}x^{8} + \frac{t_3 \left(r_3 s_2+r_2 s_3\right)}{r_3 s_3}x^{7} - \frac{\begin{gathered}
                                                                                                              r_3^2 \bigl( -s_3^2\bigr) t_2^2 +6 r_3^2 s_2^2 t_3^2 +2 r_3^2 s_3^2 t_3^2 -r_3^2 s_2 s_3 t_2 t_3 \\
                                                                                                              +13 r_2 r_3 s_2 s_3 t_3^2 -r_2 r_3 s_3^2 t_2 t_3 +6 r_2^2 s_3^2 t_3^2
                                                                                                          \end{gathered}}{4 r_3^2 s_3^2 t_3}x^{6}\notag \\
                    & \qquad{}+ \frac{\begin{gathered}
                                        \bigl(r_3 s_2 +r_2 s_3\bigr) \bigl( -3 r_3^2 s_3^2 t_2^2 +4 r_3^2 s_2^2 t_3^2 +6 r_3^2 s_3^2 t_3^2 \\
                                        -3 r_3^2 s_2 s_3 t_2 t_3 +11 r_2 r_3 s_2 s_3 t_3^2 -3 r_2 r_3 s_3^2 t_2 t_3 \\
                                        +4 r_2^2 s_3^2 t_3^2\bigr)
                                    \end{gathered}}{4 r_3^3 s_3^3 t_3}x^{5} + \sum_{i=0}^{4}c_{i,0}x^i.
\end{align}


==> text/curves/potts_mixed_full.tex <==
% Generated from notebooks/potts_mixed.nb.
% All monomials retained; c_{i,j} replaces the complete correlator-dependent coefficient.
\begin{align}
    \label{curve:potts_mixed_full}
    F_{(2)}(x,y)={} & \frac{4}{t_3^2}y^{10}{}+y^{9}\left(-\frac{4}{t_3}x^{2} - \frac{8 \left(t_2-10\right)}{t_3^2}x + \frac{8 \left(7 t_2+1\right)}{t_3^3}\right)\notag \\
                    & {}+y^{8}\left(\frac{3}{2}x^{4} + \frac{6 \left(t_2-12\right)}{t_3}x^{3} + \frac{6 \left(t_2^2-33 t_2+115\right)}{t_3^2}x^{2}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{12 \left(9 t_2^2-79 t_2-12\right)}{t_3^3}x + c_{0,8}\right)\notag \\
                    & {}+y^{7}\left(-\frac{t_3}{4}x^{6} - \frac{3}{2} \left(t_2-16\right)x^{5} - \frac{6 t_2^2-231 t_2+1109}{2 t_3}x^{4}\right.\notag \\*
                    & \qquad{}\left.{}- \frac{2 \left(t_2^3-87 t_2^2+965 t_2-1680\right)}{t_3^2}x^{3} + \sum_{i=0}^{2}c_{i,7}x^i\right)\notag \\
                    & {}+y^{6}\left(\frac{t_3^2}{64}x^{8} + \frac{1}{8} \left(t_2-28\right) t_3x^{7} + \frac{1}{8} \left(3 t_2^2-193 t_2+1291\right)x^{6}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{2 t_2^3-243 t_2^2+3621 t_2-9548}{4 t_3}x^{5} + \sum_{i=0}^{4}c_{i,6}x^i\right)\notag \\
                    & {}+y^{5}\left(\frac{3 t_3^2}{16}x^{9} + \frac{1}{16} \left(27 t_2-320\right) t_3x^{8} + \frac{1}{2} \left(12 t_2^2-311 t_2+1185\right)x^{7}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{6}c_{i,5}x^i\right)\notag \\
                    & {}+y^{4}\left(\frac{7 t_3^2}{8}x^{10} + \frac{5}{4} \left(7 t_2-48\right) t_3x^{9}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{1}{64} \left(2295 t_2^2-33210 t_2-4 t_3^2+82239\right)x^{8} + \sum_{i=0}^{7}c_{i,4}x^i\right)\notag \\
                    & {}+y^{3}\left(2 t_3^2x^{11} + 2 \left(11 t_2-50\right) t_3x^{10} + \frac{1}{8} \left(815 t_2^2-7610 t_2-4 t_3^2+13183\right)x^{9}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{8}c_{i,3}x^i\right)\notag \\
                    & {}+y^{2}\left(\frac{9 t_3^2}{4}x^{12} + \left(27 t_2-88\right) t_3x^{11}\right.\notag \\*
                    & \qquad{}\left.{}+ \frac{1}{16} \left(2227 t_2^2-14594 t_2-24 t_3^2+18524\right)x^{10} + \sum_{i=0}^{9}c_{i,2}x^i\right)\notag \\
                    & {}+y\left(t_3^2x^{13} + \left(13 t_2-32\right) t_3x^{12} + \frac{1}{4} \left(295 t_2^2-1434 t_2-8 t_3^2+1376\right)x^{11}\right.\notag \\*
                    & \qquad{}\left.{}+ \sum_{i=0}^{10}c_{i,1}x^i\right)\notag \\
                    & {}-t_3^2x^{12} + \sum_{i=0}^{11}c_{i,0}x^i.
\end{align}

